Radio relics radio emission from multi-shock scenario

Radio relics are giant ($\sim$Mpc) synchrotron sources that are believed to be produced by the (re)acceleration of cosmic-ray electrons (CRe) by shocks in the intracluster medium. In this numerical study, we focus on the possibility that some radio relics may arise when electrons undergo diffusive shock acceleration at multiple shocks in the outskirts of merging galaxy clusters. This multi-shock (MS) scenario appears viable to produce CRe that emit visible synchrotron emission. We show that electrons that have been shocked multiple times develop an energy spectrum that significantly differs from the power-law spectrum expected in the case of a single shock scenario. As a consequence, the radio emission generated by CRe that shocked multiple times is higher than the emission produced by CRe that are shocked only once. In the case explored in this paper, the radio emission produced in the two scenarios differ by one order of magnitude. In particular in the MS scenario, the simulated relic follows a KGJP spectral shape, consistent with observation. Furthermore, the produced radio emission is large enough to be detectable with current radio telescopes (e.g. LOFAR, JVLA).

==> commands.tex <==
\newcommand{\aaps}{Astronomy and Astrophysics Supplement}
\newcommand{\apss}{APSS}
\newcommand{\apjs}{ApJS}
\newcommand{\apj}{ApJ}
\newcommand{\aj}{ApJ}
\newcommand{\apjl}{ApJ Letters}
\newcommand{\mnras}{MNRAS}
\newcommand{\aap}{A\&A}
\newcommand{\ETC}{et al.}
\newcommand{\ssr}{Science \& Space Review}
\newcommand{\na}{New Astronomy}
\newcommand{\nat}{Nature}
\newcommand{\physrep}{Physics Reports}
\newcommand{\aapr}{The Astronomy and Astrophysics Review}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\pasp}{Publication of the Astronomical Society of the Pacific}
\newcommand{\prd}{Physical Review Letters}
\newcommand{\jgr}{Journal of Geophysical Research}
\newcommand{\pasa}{Publications of the Astronomical Society of Australia}
\newcommand{\pasj}{Publications of the Astronomical Society of Japan}
\newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
\newcommand{\enzo}{\textsc{ENZO}}
\newcommand{\CRaTer}{\textsc{CRaTer}}
\newcommand{\flash}{{\it {\small Flash}}}
\newcommand{\music}{{\it {\small MUSIC}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\Msun}{\mathrm{M}_{\odot}}
\newcommand{\Mth}{\mathrm{M}_{200}}
\newcommand{\rth}{\mathrm{r}_{200}}
\newcommand{\kpc}{\mathrm{kpc}}
\newcommand{\radio}{\mathrm{radio}}
\newcommand{\ph}{\mathrm{ph}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\km}{\mathrm{km}}
\newcommand{\sek}{\mathrm{s}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\K}{\mathrm{K}}
\newcommand{\Gyr}{\mathrm{Gyr}}
\newcommand{\Myr}{\mathrm{Myr}}
\newcommand{\all}{\mathrm{all}}
\newcommand{\para}{\mathrm{para}}
\newcommand{\erg}{\mathrm{erg}}
\newcommand{\Hz}{\mathrm{Hz}}
\newcommand{\MHz}{\mathrm{MHz}}
\newcommand{\GHz}{\mathrm{GHz}}
\newcommand{\pre}{\mathrm{pre}}
\newcommand{\post}{\mathrm{post}}
\newcommand{\fc}{F_{\mathrm{comp}}}
\newcommand{\fst}{F_{\mathrm{stretch}}}
\newcommand{\fb}{F_{\mathrm{baro}}}
\newcommand{\fdiss}{F_{\mathrm{diss}}}
\newcommand{\fadv}{F_{\mathrm{adv}}}
\newcommand{\nuobs}{\nu_{\mathrm{obs}}}
\newcommand{\Pburn}{P_{\mathrm{Burn}}}
\newcommand{\Ptot}{P_{\mathrm{tot}}}
\newcommand{\Ppara}{P_{\mathrm{\perp}}}
\newcommand{\Pperp}{P_{\mathrm{\parallel}}}
\newcommand{\Csync}{C_{\mathrm{sync}}}
\newcommand{\Cspec}{C_{\mathrm{spec}}}
\newcommand{\Ctau}{C_{\tau}}
\newcommand{\burn}{\mathrm{Burn}}
\newcommand{\rad}{\mathrm{rad}}
\newcommand{\asec}{\mathrm{arcsec}}
\newcommand{\m}{\mathrm{m}}
\newcommand{\Jy}{\mathrm{Jy}}
\newcommand{\beam}{\mathrm{beam}}
\newcommand{\RM}{\mathrm{RM}}
\newcommand{\vvec}{\mathbf{v}}
\newcommand{\pc}{\mathbf{pc}}
\newcommand{\me}{m_\mathrm{e}}
\newcommand{\mpr}{m_\mathrm{p}}
\newcommand{\gram}{\mathrm{g}}
\newcommand{\aint}{\alpha_{\mathrm{int}}}
\newcommand{\ainj}{\alpha_{\mathrm{inj}}}
\newcommand{\alow}{\alpha_{\mathrm{low}}}
\newcommand{\ahigh}{\alpha_{\mathrm{high}}}



==> radio relics multiple shocks/commands.tex <==
\newcommand{\aaps}{Astronomy and Astrophysics Supplement}
\newcommand{\apss}{APSS}
\newcommand{\apjs}{ApJS}
\newcommand{\apj}{ApJ}
\newcommand{\aj}{ApJ}
\newcommand{\apjl}{ApJ Letters}
\newcommand{\mnras}{MNRAS}
\newcommand{\aap}{A\&A}
\newcommand{\ETC}{et al.}
\newcommand{\ssr}{Science \& Space Review}
\newcommand{\na}{New Astronomy}
\newcommand{\nat}{Nature}
\newcommand{\physrep}{Physics Reports}
\newcommand{\aapr}{The Astronomy and Astrophysics Review}
\newcommand{\jcap}{Journal of Cosmology and Astroparticle Physics}
\newcommand{\pasp}{Publication of the Astronomical Society of the Pacific}
\newcommand{\prd}{Physical Review Letters}
\newcommand{\jgr}{Journal of Geophysical Research}
\newcommand{\pasa}{Publications of the Astronomical Society of Australia}
\newcommand{\pasj}{Publications of the Astronomical Society of Japan}
\newcommand{\araa}{Annual Review of Astronomy and Astrophysics}
\newcommand{\enzo}{\textsc{ENZO}}
\newcommand{\CRaTer}{\textsc{CRaTer}}
\newcommand{\flash}{{\it {\small Flash}}}
\newcommand{\music}{{\it {\small MUSIC}}}
\newcommand{\dd}{\mathrm{d}}
\newcommand{\Mpc}{\mathrm{Mpc}}
\newcommand{\Msun}{\mathrm{M}_{\odot}}
\newcommand{\Mth}{\mathrm{M}_{200}}
\newcommand{\rth}{\mathrm{r}_{200}}
\newcommand{\kpc}{\mathrm{kpc}}
\newcommand{\radio}{\mathrm{radio}}
\newcommand{\ph}{\mathrm{ph}}
\newcommand{\cm}{\mathrm{cm}}
\newcommand{\km}{\mathrm{km}}
\newcommand{\sek}{\mathrm{s}}
\newcommand{\keV}{\mathrm{keV}}
\newcommand{\MeV}{\mathrm{MeV}}
\newcommand{\GeV}{\mathrm{GeV}}
\newcommand{\eV}{\mathrm{eV}}
\newcommand{\TeV}{\mathrm{TeV}}
\newcommand{\G}{\mathrm{G}}
\newcommand{\K}{\mathrm{K}}
\newcommand{\Gyr}{\mathrm{Gyr}}
\newcommand{\Myr}{\mathrm{Myr}}
\newcommand{\all}{\mathrm{all}}
\newcommand{\para}{\mathrm{para}}
\newcommand{\erg}{\mathrm{erg}}
\newcommand{\Hz}{\mathrm{Hz}}
\newcommand{\MHz}{\mathrm{MHz}}
\newcommand{\GHz}{\mathrm{GHz}}
\newcommand{\pre}{\mathrm{pre}}
\newcommand{\post}{\mathrm{post}}
\newcommand{\fc}{F_{\mathrm{comp}}}
\newcommand{\fst}{F_{\mathrm{stretch}}}
\newcommand{\fb}{F_{\mathrm{baro}}}
\newcommand{\fdiss}{F_{\mathrm{diss}}}
\newcommand{\fadv}{F_{\mathrm{adv}}}
\newcommand{\nuobs}{\nu_{\mathrm{obs}}}
\newcommand{\Pburn}{P_{\mathrm{Burn}}}
\newcommand{\Ptot}{P_{\mathrm{tot}}}
\newcommand{\Ppara}{P_{\mathrm{\perp}}}
\newcommand{\Pperp}{P_{\mathrm{\parallel}}}
\newcommand{\Csync}{C_{\mathrm{sync}}}
\newcommand{\Cspec}{C_{\mathrm{spec}}}
\newcommand{\Ctau}{C_{\tau}}
\newcommand{\burn}{\mathrm{Burn}}
\newcommand{\rad}{\mathrm{rad}}
\newcommand{\asec}{\mathrm{arcsec}}
\newcommand{\m}{\mathrm{m}}
\newcommand{\Jy}{\mathrm{Jy}}
\newcommand{\beam}{\mathrm{beam}}
\newcommand{\RM}{\mathrm{RM}}
\newcommand{\vvec}{\mathbf{v}}
\newcommand{\pc}{\mathbf{pc}}
\newcommand{\me}{m_\mathrm{e}}
\newcommand{\mpr}{m_\mathrm{p}}
\newcommand{\gram}{\mathrm{g}}
\newcommand{\aint}{\alpha_{\mathrm{int}}}
\newcommand{\ainj}{\alpha_{\mathrm{inj}}}
\newcommand{\alow}{\alpha_{\mathrm{low}}}
\newcommand{\ahigh}{\alpha_{\mathrm{high}}}


